JADES: Using NIRCam Photometry to Investigate the Dependence of Stellar Mass Inferences on the IMF in the Early Universe

The detection of numerous and relatively bright galaxies at redshifts z > 9 has prompted new investigations into the star-forming properties of high-redshift galaxies. Using local forms of the initial mass function (IMF) to estimate stellar masses of these galaxies from their light output leads to galaxy masses that are at the limit allowed for the state of the LambdaCDM Universe at their redshift. We explore how varying the IMF assumed in studies of galaxies in the early universe changes the inferred values for the stellar masses of these galaxies. We infer galaxy properties with the SED fitting code Prospector using varying IMF parameterizations for a sample of 102 galaxies from the JWST Advanced Deep Extragalactic Survey (JADES) spectroscopically confirmed to be at z > 6.7, with additional photometry from the JWST Extragalactic Medium Band Survey (JEMS) for twenty-one galaxies. We demonstrate that models with stellar masses reduced by a factor of three or more do not affect the modeled spectral energy distribution (SED).

==> orcids_for_pnas.tex <==
% PNAS strongly encourages authors to supply an ORCID identifier for each author. Do not include ORCIDs in the manuscript file; individual authors must link their ORCID account to their PNAS account at www.pnascentral.org. For proper authentication, authors must provide their ORCID at submission and are not permitted to add ORCIDs on proofs.

Charity Woodrum: 0000-0001-5962-7260
Marcia Rieke: 0000-0002-7893-6170
Zhiyuan Ji: 0000-0001-7673-2257

William M. Baker: 0000-0003-0215-1104
Rachana Bhatawdekar: 0000-0003-0883-2226
Andrew J. Bunker: 0000-0002-8651-9879
Stefane Charlot: 0000-0003-3458-2275
Emma Curtis-Lake: 0000-0002-9551-0534
Daniel J. Eisenstein: 0000-0002-2929-3121
Kevin Hainline: 0000-0003-4565-8239
Ryan Hausen: 0000-0002-8543-761X
Jakob M. Helton: 0000-0003-4337-6211
Raphael H. Hviding: 0000-0002-4684-9005
Benjamin D. Johnson: 0000-0002-9280-7594
Brant Robertson: 0000-0002-4271-0364
Fengwu Sun: 0000-0002-4622-6617
Sandro Tacchella: 0000-0002-8224-4505
Lily Whitler: 0000-0003-1432-7744
Christina C. Williams: 0000-0003-2919-7495
Christopher N.A. Willmer: 0000-0001-9262-9997
